Shape-aware Text-driven Layered Video Editing

Temporal consistency is essential for video editing applications. Existing work on layered representation of videos allows propagating edits consistently to each frame. These methods, however, can only edit object appearance rather than object shape changes due to the limitation of using a fixed UV mapping field for texture atlas. We present a shape-aware, text-driven video editing method to tackle this challenge. To handle shape changes in video editing, we first propagate the deformation field between the input and edited keyframe to all frames. We then leverage a pre-trained text-conditioned diffusion model as guidance for refining shape distortion and completing unseen regions. The experimental results demonstrate that our method can achieve shape-aware consistent video editing and compare favorably with the state-of-the-art.

==> figures/fig_supp_additional_visual_results.tex <==
\begin{figure*}[h]
    \centering
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/input/00010.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/input/00020.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/input/00030.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/input/00040.png}} \\
    \vspace{0.1cm}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/output/00010.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/output/00020.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/output/00030.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/swan/output/00040.png}} \\
    ``\texttt{black swan}~\textrightarrow~\texttt{white swan}'' + ``\texttt{river}~\textrightarrow~\texttt{cartoon-style river}'' \\
    \vspace{0.3cm}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/input/00005.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/input/00015.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/input/00025.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/input/00035.png}} \\
    \vspace{0.1cm}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/output/00005.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/output/00015.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/output/00025.png}}
    \frame{\includegraphics[width=0.245\linewidth]{figures/additional_visual/surf/output/00035.png}} \\
    ``\texttt{surfing}~\textrightarrow~\texttt{sail boat}'' + ``\texttt{sea}~\textrightarrow~\texttt{cartoon-style sea with strong wave}'' \\
    \caption{\textbf{Additional visual results with foreground and background editing.}}
    \label{fig:supp_visual_results}
\end{figure*}

==> figures/fig_supp_edit_bg_atlas.tex <==
\begin{figure}
    \centering
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{\hspace{0.4cm}Atlas}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_input/atlas.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example1/atlas.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example2/atlas.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example3/atlas.png}} \\
    \vspace{-1.38cm}
    \hline
    \vspace{0.1cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{$\longleftarrow$ time}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/00025.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example1/00025.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example2/00025.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example3/00025.png}} \\
    \vspace{-1.5cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/00040.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example1/00040.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example2/00040.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example3/00040.png}} \\
    \vspace{-0.85cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/00055.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example1/00055.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example2/00055.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/bg_example3/00055.png}} \\
    \vspace{-0.9cm}
    \caption{\textbf{Editing on background atlases.} The source and edited background atlases are shown in the top row, and the resulting frames are in the same column. The background atlas can be treated as a natural panorama image for image editing. In addition, the edited background atlases can be directly used for the entire video since each visible pixel is edited in atlases.}
    \label{fig:supp_edit_bg_atlas}
\end{figure}

==> figures/fig_supp_edit_fg_atlas.tex <==
\begin{figure}
    \centering
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{\hspace{1.8cm}Atlas}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/atlas.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example1/atlas.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example2/atlas.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example3/atlas.png}} \\
    \vspace{-2.1cm}
    \hline
    \vspace{0.1cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{$\longleftarrow$ time}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/00025.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example1/00025.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example2/00025.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example3/00025.png}} \\
    \vspace{-1.5cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/00040.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example1/00040.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example2/00040.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example3/00040.png}} \\
    \vspace{-0.85cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{}}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_input/00055.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example1/00055.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example2/00055.png}}
    \frame{\includegraphics[width=0.23\linewidth]{figures/edit_atlas/fg_example3/00055.png}} \\
    \vspace{-0.9cm}
    \caption{\textbf{Editing on foreground atlases.} The source and edited foreground atlases are demonstrated in the top row, and the resulting frames are in the same column. The foreground atlas is an unwrapped texture due to the 3D object motion in the video. The distorted atlas poses a challenge for the general pre-trained Stable Diffusion to manipulate. As a result, the artifacts are shown in the rendered frames because of the incomplete and distorted edited atlases.}
    \label{fig:supp_edit_fg_atlas}
\end{figure}

==> figures/fig_supp_editing_image_and_atlas.tex <==
\begin{figure*}
    \centering
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{\hspace{-0.3cm}Image}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/image_input.png}}
    \unskip\ \vrule height 1.9cm depth 2cm \ 
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/image01.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/image02.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/image03.png}}\\
    \vspace{-2.05cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{\hspace{1.4cm}FG atlas}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/atlas_input.png}}
    \unskip\ \vrule height 4cm depth 0.cm \ 
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/atlas01.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/atlas02.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/atlas03.png}}\\
    \vspace{-2.4cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{BG atlas}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/bg_input.png}}
    \unskip\ \vrule height 2.2cm depth 0.cm \ 
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/bg02.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/bg01.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/difference_editing/bg03.png}}\\
    \vspace{-1.5cm}
    \caption{\textbf{Editing on foreground atlases.}}
    \label{fig:supp_editing_image_and_atlas}
\end{figure*}

==> figures/fig_supp_text2live_variant.tex <==
\begin{figure*}
    \centering
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{Input}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/teaser/input/00036.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/teaser/input/00042.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/teaser/input/00048.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/teaser/input/00054.png}} \\
    \vspace{-1.175cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{Ours}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/ours/00036.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/ours/00042.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/ours/00048.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/ours/00054.png}} \\
    \vspace{-1.15cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{Text2LIVE~\cite{bar2022text2live}}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live/00036.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live/00042.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live/00048.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live/00054.png}} \\
    \vspace{-1.85cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{\small{\cite{bar2022text2live} w/o struct.}}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_wo_structure/00036.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_wo_structure/00042.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_wo_structure/00048.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_wo_structure/00054.png}} \\
    \vspace{-1.825cm}
    \mpage{0.02}{\raisebox{2cm}{\rotatebox{90}{\small{\cite{bar2022text2live} w/ trained UV}}}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_w_trained_uv/00036.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_w_trained_uv/00042.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_w_trained_uv/00048.png}}
    \frame{\includegraphics[width=0.22\linewidth]{figures/visual_comparison/sports/text2live_w_trained_uv/00054.png}} \\
    \vspace{-2.3cm}
    \caption{\textbf{Visual comparison with modified Text2LIVE~\cite{bar2022text2live}.} We attempt to modify the official Text2LIVE to enable shape-aware editing. We remove the shape preservation loss, but the results still remain in the source shape due to the fixed UV (as in the 4\textsuperscript{th} row, w/o struct.) Therefore, we further try to jointly train the per-frame UV maps during the optimization. However, the training of UV maps makes noisy and temporal flickering in the 5\textsuperscript{th} row, w/ trained UV). In sum, we believe that Text2LIVE is not feasible for shape-aware editing.}
    \label{fig:supp_text2live_variant}
\end{figure*}

==> figures/fig_supp_user_study.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/user-study/figure.pdf}
    \caption{\textbf{Quantitative comparison by human evaluation.} We show the users' judgment of our method with each of compared baseline methods and Text2LIVE~\cite{bar2022text2live}. In general, most participants prefer our method to other approaches.}
    \label{fig:supp_user_study}
\end{figure}
